Textual Training for the Hassle-Free Removal of Unwanted Visual Data: Case Studies on OOD and Hateful Image Detection

In our study, we explore methods for detecting unwanted content lurking in visual datasets. We provide a theoretical analysis demonstrating that a model capable of successfully partitioning visual data can be obtained using only textual data. Based on the analysis, we propose Hassle-Free Textual Training (HFTT), a streamlined method capable of acquiring detectors for unwanted visual content, using only synthetic textual data in conjunction with pre-trained vision-language models. HFTT features an innovative objective function that significantly reduces the necessity for human involvement in data annotation. Furthermore, HFTT employs a clever textual data synthesis method, effectively emulating the integration of unknown visual data distribution into the training process at no extra cost. The unique characteristics of HFTT extend its utility beyond traditional out-of-distribution detection, making it applicable to tasks that address more abstract concepts. We complement our analyses with experiments in out-of-distribution detection and hateful image detection. Our codes are available at https://github.com/Saehyung-Lee/HFTT

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}
%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Abstract and Section 1
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 5
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 3 and Appendix A
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: URL in Abstract and Section 4
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: URL in Abstract
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: URL in Abstract and Section 4
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We report the results over five runs. The variances of the results are close to zero so reporting them would be redundant.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 4.1
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our submission conform, in every respect, with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 5
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not release any data or model.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 4 and Appendix
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: URL in abstract and Section 4
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> main/rebuttal.tex <==
We genuinely appreciate the reviewers' dedicated time and their valuable feedback. Before addressing each reviewer's specific concerns in detail below, we would like to summarize here the contributions of our research that have been recognized and the aspects that have been enhanced in our study.
## Acknowledgement of Our Contributions by Reviewers
- The theoretical justification of our proposed method is solid (CzuR, LurW).
- We demonstrate that it is possible to obtain an effective unwanted image detector without using images (CzuR, QxHY, kqnV).
- Our method is innovative, efficient, effective, and useful in practice (CzuR, LurW, QxHY, kqnV). 
- The experiments are comprehensive, and the results show the effectiveness of our proposed method (LurW, kqnV).
- For the reproducibility of our method, we provide a cost analysis, implementation details, and code (LurW, kqnV).

## Enhancements in Our Paper
- We provide additional discussion on the comparison with state-of-the-art OOD detection methods.
- We present comparative results against NegLabel and CLIPN in the medical image domain.
- We offer experimental results and discussion regarding other foundation models, such as BLIP.
- We provide a discussion on the application of our method to multi-class classification tasks.

We provide detailed responses to each reviewer's comments below. We have diligently addressed each of the four reviewers' concerns to the best of our abilities, and believe that the results further underscore the contributions of our study. We plan to integrate the reviewers' suggestions into the revisions of the manuscript, as we believe these adjustments will significantly bolster the paper's overall strength.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Response to Reviewer CzuR


Firstly, we express our gratitude for your thorough review of our manuscript. Particularly, we appreciate your recognition of our method as valuable and useful in practice, as well as your acknowledgment that the justification of our method is well-motivated and clearly presented. Furthermore, we appreciate your invaluable suggestions, which significantly enrich the substance of our work. In the subsequent sections, we meticulously address each of your concerns as follows:

>**W1**. The related work section lacks comprehensiveness. While the authors mention some CLIP-based methods, they overlook approaches closely related to their own. Notably, NegLabel (ICLR2024) and CLIPN (ICCV2023) also use textual features for OOD detection and are very similar to the proposed method. The authors should include these works in their related work section, provide benchmarks, and critically analyze the advantages of their approach compared to these existing methods.

**A1**. Thank you for your feedback on the two related studies. We can compare our method with each of these studies as follows. This discussion will be added to the final version of our paper:

**Comparison with NegLabel**  
NegLabel constructs an OOD corpus by selecting texts distant from the in-distribution texts from a predefined corpus, then compares the distances between the input image and those texts in the CLIP embedding space to detect OOD. While NegLabel shows high OOD detection performance on ImageNet (see Table B), it has the following limitations compared to our method:
- Although NegLabel does not require training additional parameters, it must compute the embeddings of all texts in the corpus and measure their similarity to the in-distribution texts to find the optimal OOD corpus for a given in-distribution. Our training method also requires nearly the same cost as obtaining the embeddings of all texts within a predefined corpus and calculating the similarities between those embeddings and the task+trainable embeddings, as discussed in Section 4.1. Thus, NegLabel and our method require the same level of optimization cost.
- Since NegLabel uses the embeddings of the determined OOD corpus as they are, it falls behind our method, which has trainable parameters, in terms of generalization. To demonstrate this, we further compare our method and NegLabel in the medical image domain. Specifically, we treat the ISIC-18 skin lesion diagnosis dataset [1] as in-distribution and the PathVQA [2] and PatchCamelyon [3] datasets as out-of-distribution. The ISIC-18 skin lesion diagnosis dataset is an image classification benchmark for seven skin disease categories.

Table A: OOD detection in the medical image domain
|    OOD:   | PVQA | | PCAM | |
| ----------------- | ----- | ----- | ----- | ----- |
| **Method**     | **FPR** &#8595; | **AUROC** &#8593; | **FPR** &#8595; | **AUROC** &#8593; |
| NegLabel    | 37.44   | 94.11   |48.07   | 94.86   |
| CLIPN  | 35.47   |  84.64  |3.10   | 98.76   |
| HFTT (ours)   | 13.72   | 97.05   |4.95   | 98.35   |

Table A illustrates the limitations of NegLabel in terms of generalization. While NegLabel fails to construct an effective OOD corpus for the medical image dataset, our method achieves significantly higher performance by learning optimal embeddings for detection.

**Comparison with CLIPN**  
CLIPN utilizes an additional "no" text encoder alongside CLIP. This additional text encoder predicts the probability that a given object is not present in an image. Thus, CLIPN predicts whether a given image is in-distribution or out-distribution by using the original CLIP text encoder and the "no" text encoder to estimate the probabilities, respectively. Images with a low probability of being in-distribution and a high probability of being out-distribution are identified as OOD.

Although CLIPN achieves high OOD detection performance on ImageNet (see Table B), it has the following limitations compared to our method:

- CLIPN requires significantly higher inference costs due to the use of an additional text encoder.
- While our method requires lightweight training that does not involve images, CLIPN demands extensive and expensive training of the "no" text encoder on large vision-language datasets.
- CLIPN can only be applied to tasks where the distinction between in-distribution and out-distribution is clear and straightforward, such as classification datasets. This is because all training images must be classified as either "yes" or "no" images. Therefore, it is unsuitable for tasks dealing with abstract concepts, such as hateful image detection, as discussed in Section 4.3 of our paper.
- Our method can be easily applied to any detection task defined in natural language, whereas CLIPN shows significantly degraded performance for in-distribution tasks that fall outside the training distribution of the "no" text encoder. In terms of applicability, our proposed method surpasses CLIPN. To demonstrate this, we further compare our method with CLIPN in the medical image domain. Table A illustrates the limitations of CLIPN in terms of generalization. While CLIPN effectively detects PCAM, it exhibits very low detection performance on PVQA. In contrast, our method achieves high performance on both OOD tasks.

Table B: OOD detection performance on ImageNet in-distribution (average for Texture, Places, SUN, and iNaturalist)
| OOD:  | Average ||
| ----------------- | ----- | ----- |
| **Method**            | **FPR** &#8595; | **AUROC** &#8593; |
| CLIPN    | 31.10   | 93.10 |
| NegLabel  | 25.40  |  94.21 |
| HFTT (ours)   | 33.33   | 91.76 |

[1] Codella, Noel, et al. "Skin lesion analysis toward melanoma detection 2018: A challenge hosted by the international skin imaging collaboration (isic)." arXiv 2019.  
[2] He, Xuehai, et al. "Pathvqa: 30000+ questions for medical visual question answering." arXiv 2020.  
[3] Veeling, Bastiaan S., et al. "Rotation equivariant CNNs for digital pathology." MICCAI 2018.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

>**W2**. In the experimental results, authors compare results with CLIPN and NegLabel only in Tab. 2, while they are not mentioned in Tab.1. Also, those two methods are not even cited nor explained in related work. I believe it might have been a last minute effort.

**A2**. We apologize for not adequately introducing the two studies. During this rebuttal period, we have made our best efforts to compare the two methods with our own, and we provided this discussion in **A1**. The above discussion will be added to the Related Work and Experimental Results and Discussion sections of the main text.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

>**W3**. Some methods in the literature do not require any training (e.g. NegLabel). Given that the proposed approach involves additional training (even though without images), it is crucial to highlight the differences with these training-free methods.

**A3**. NegLabel does not require training but demands a process to find the optimal OOD corpus for a given in-distribution. This process involves obtaining the embeddings of all texts within a predefined corpus, calculating their similarities to the in-distribution texts, and constructing an embedding set that is the most distant yet diverse from the in-distribution. Our training method, as discussed in Section 4.1 of the main text, also requires nearly the same cost of obtaining the embeddings of all texts within a predefined corpus and calculating the similarities between those embeddings and task+trainable embeddings. Therefore, we can say that our method and NegLabel require the same level of cost. Additionally, as discussed in **A1**, our method, which has trainable parameters, may be advantageous in terms of generalization compared to NegLabel, which uses predefined embeddings.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Official Review of Submission3444 by Reviewer LurW

Firstly, we thank you for your thorough review of our paper. We particularly appreciate your recognition that our paper has no significant weaknesses and is well-organized. We have made our best efforts to address your remaining concerns as follows. If our responses meet your expectations, we would be grateful if you could consider reflecting this in your evaluation:

>**Q1**. This idea of training on textual content for transferring to visual content is interesting, could the authors provide more insights on more examples of applications of this method except for the OOD detection and hateful image detection? Is it possible to apply it to more binary classification tasks?

**A1**. Our method can be applied to more binary classification tasks. We additionally demonstrate the applicability of our method, HFTT, in detecting low-quality images, which are commonly unwanted visual data beyond OOD and hate images. Specifically, we assume the task of detecting corrupted images lurking within a raw visual dataset consisting of 1000 ImageNet classes. For this experiment, we use ImageNet and ImageNet-C. As shown in Table A below, HFTT consistently surpasses existing methods in the detection of corrupted images.

Table A: Corrupted image detection
| Method            | FPR &#8595; | AUROC &#8593; |
| - | - | - |
| MSP | 64.17   | 83.94   |
| Energy | 99.99   |  09.16  |
| MaxLogit  | 78.01   | 68.47   |
| MCM    | 51.54   | 89.06   |
| HFTT (ours)   | **42.13**   | **92.81**   |

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

>**Q2**. What encoders are used to obtain the task embedding? The authors mentioned using CLIP as the vision backbone, and is the text encoder during training also from CLIP?

**A2**. As discussed in Section 3.1 of our paper, our method assumes that text and image are well-aligned through contrastive learning, similar to CLIP. Therefore, if CLIP is used as the vision encoder, the text encoder must also be CLIP. If text and image are well-aligned, our method can be applied to models other than CLIP. To demonstrate this, we additionally apply our method to BLIP and observe the results. Table B shows that our method is also effective for BLIP.

Table B: The experimental results on BLIP
| OOD:  | iNaturalist || SUN ||  Places || Texture || NINCO || 
| - | - | - | - | - | - | - | - | - | - | - |
| **Method**            | **FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |
| MSP |  64.70 | 82.22 | 30.38 | 91.06 | 71.40 | 78.82 | 76.99 | 81.30 | **71.47** | 72.07   |
| Energy | 67.15 |  79.30 |  45.21 |  89.07 |  70.28  | 77.49 |  91.24 |  75.38 |  80.29  | **77.20**  |
| MaxLogit |  69.57 | 75.44 | 69.57 | 71.19 | 69.86 | 76.26 | 93.55 | 60.31 | 88.58 | 56.37 |
| MCM| 64.41  | **82.29** | 30.21 | 91.05 | 70.53 | 79.32 | 75.84 | 81.55 | 71.56 | 72.02  |
| HFTT (ours)    | **63.28** | 82.22 | **19.16** | **95.12** | **68.48** | **79.50** | **63.74** | **84.53** | 72.12 | 73.86   |



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

>**Q3**. How do you decide the number of task embeddings?

**A3**. The number of task embeddings is not a hyper-parameter but is determined by the in-distribution task. For example, if the in-distribution is ImageNet, the task embeddings are the text embeddings for the 1,000 ImageNet classes, such as ["a photo of a tench", ..., "a photo of a toilet paper"]. In the case of hateful image detection, we used representative hate phrases defined by the dataset as task embeddings. The number of trainable embeddings in our method is a hyper-parameter. We present an ablation study on this in Table 8 of Appendix C, and the results show that our method is not sensitive to this parameter.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

>**Q4**. The paper mentions using the proposed method to detect unwanted content and uses two tasks (OOD detection and hateful image detection. If I understand correctly, my key concern is that the focus of this paper is closer to a novel method for binary classification with an application that classifies unwanted content. Could the authors share more thoughts regarding this? If so, I would suggest slightly paraphrasing the introduction to better reflect the contribution and indicate more potential applications.

**A4**. We are hesitant to consider our method as a novel approach for binary classification. Generally, binary classification is defined as the task of finding patterns that best distinguish between two different classes. However, in our scenario, we assume that only one (in-distribution) of the two classes has patterns, while we make no assumptions about the other class to cover all possible cases. Therefore, for binary classification tasks where both classes have specific patterns, our method may not lead to a good solution compared to methods that consider patterns of both classes. Thus, we would like to distinguish our method from general binary classification methods. We appreciate the reviewer for prompting us to view our method in this light.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

>**Q5**. Can this method be extended to multi-class classifications?

**A5**. In fact, our proposed method can always perform multi-class classification and unwanted data detection simultaneously. Figure 1 in our paper or the figure in our repository (https://github.com/HFTT-anonymous/HFTT) can aid in understanding this. HFTT utilizes the input embeddings and logit values as they are for zero-shot classification while simultaneously estimating the probability that an input sample is unwanted. For example, our method can be applied to solve a 1001-class classification task consisting of 1000 ImageNet classes plus one OOD class.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Official Review of Submission3444 by Reviewer QxHY

Firstly, we thank you for your thorough review of our paper. We particularly appreciate your recognition that our method is the compelling approach of utilizing text-only mode for detecting data in other modes and that the training and inference processes are highly efficient. We are also immensely grateful for your excellent suggestions that can enhance the contents of our paper. We will address each of your concerns in detail in the following:

>**Q1**. The trainable embedding learning process is unclear. According to the description, trainable embeddings are learned for N out-distribution data instances, which are then frozen during the test phase. It appears that the image embeddings obtained by the image encoder align with the frozen embeddings. If this is the case, the alignment process should be clearly elucidated. If not, the method for using the learned embeddings for images needs to be explained. 

**A1**. In Section 3.1 of our paper, we presented a motivating example demonstrating that a classifier obtained using only textual data in the output space of a model like CLIP, where images and texts are well-aligned, can also be applied to image data. Based on this, we proceed as follows:
1. We define trainable embeddings in the output space of CLIP that serve as the parameters of a classifier distinguishing between in-distribution and out-distribution data.
2. We train these embeddings using only textual data.
3. We use these trained embeddings to detect unwanted images.
In summary, the model parameters of CLIP remain fixed, and our trainable parameters are defined and trained within CLIP’s (image-text) joint embedding space. Thus, our method does not require any additional alignment process.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

>**Q2**. The parameter N, representing the number of out-distribution data used during training, intuitively suggests that a larger N would enhance accurate distribution learning. However, the results in Table 8 present a contradictory viewpoint. More explanation should be given.

**A2**. We apologize for any confusion caused by our notation. The "N" in Table 8 refers to the number of trainable embeddings, not the number of out-distribution data. The number of trainable embeddings in our method represents the complexity of the classifier that distinguishes between in-distribution and out-distribution data. If the data in CLIP's output space form a very low-dimensional manifold, it would be possible to distinguish between in- and out-distribution data with a small number of trainable embeddings. As we can see in Table 8, a large "N" is not necessary for high unwanted image detection results. Indeed, various studies support the notion that deep learning models possess low-dimensional data manifolds [1,2].

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

>**Q3**. The test on other pre-trained models to view how the pre-learned cross-modal alignment knowledge impacts the text-only learning.

**A3**. Thank you very much for suggesting an expansion of our research domain. Video embedding models and detection tasks are less established than those in the image domain. We will investigate the experimental environment further and include results in the next version of our paper. Here, we provide the results for CLIP-L/14, BLIP-B/16, and BLIP-L/16 in addition to the CLIP-B/16 used in our study. Tables A, B, and C demonstrate that our method is effective across various vision-language models.

Table A: The experimental results on CLIP-L/14 (in-distribution: ImageNet)
| OOD:  | iNaturalist || SUN ||  Places || Texture || NINCO || 
| - | - | - | - | - | - | - | - | - | - | - |
| **Method**            | **FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |
| MSP |   26.66| 94.20| 22.37| 94.37| 36.82| 92.45| 52.83| 86.57| 67.27| 78.70  |
| Energy | 30.84 |91.25 |25.94 |94.10 |32.94 |92.30 |64.33 |79.26 |63.49 |79.72   |
| MaxLogit |  32.76| 90.96 |26.48| 92.96| **31.88**| 92.39| 72.08| 73.85| **60.67**| **81.07** |
| MCM| 64.41  | 26.96 |94.19 |22.77 |94.37 |36.74 |92.44 |52.66 |86.56 |68.16 |78.65  |
| HFTT (ours)    | **24.10**| **94.58**| **17.80**| **95.39**| 33.83| **93.09**| **52.06**| **86.58**| 69.19| 78.98    |

Table B: The experimental results on BLIP-B/16 (in-distribution: ImageNet)
| OOD:  | iNaturalist || SUN ||  Places || Texture || NINCO || 
| - | - | - | - | - | - | - | - | - | - | - |
| **Method**            | **FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |
| MSP |  64.70 | 82.22 | 30.38 | 91.06 | 71.40 | 78.82 | 76.99 | 81.30 | **71.47** | 72.07   |
| Energy | 67.15 |  79.30 |  45.21 |  89.07 |  70.28  | 77.49 |  91.24 |  75.38 |  80.29  | **77.20**  |
| MaxLogit |  69.57 | 75.44 | 69.57 | 71.19 | 69.86 | 76.26 | 93.55 | 60.31 | 88.58 | 56.37 |
| MCM| 64.41  | **82.29** | 30.21 | 91.05 | 70.53 | 79.32 | 75.84 | 81.55 | 71.56 | 72.02  |
| HFTT (ours)    | **63.28** | 82.22 | **19.16** | **95.12** | **68.48** | **79.50** | **63.74** | **84.53** | 72.12 | 73.86   |

Table C: The experimental results on BLIP-L/16 (in-distribution: ImageNet)
| OOD:  | iNaturalist || SUN ||  Places || Texture || NINCO || 
| - | - | - | - | - | - | - | - | - | - | - |
| **Method**            | **FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |
| MSP |   51.20| 87.91| 22.37| 93.86| 61.63| 84.68| 64.85| 85.28| 65.96| 78.29 |
| Energy | 45.63 |87.23 |33.94 |90.29 |55.73 |85.91 |72.38 |82.16 |71.23| 77.49  |
| MaxLogit |  44.59| 86.94| 35.56| 86.45| **50.96**| **86.46**| 86.38| 71.22| 79.78| 67.59  |
| MCM| 50.75 |88.03 |22.34 |93.88 |60.88 |85.38 |64.71 |**85.39** |66.04| 78.32  |
| HFTT (ours)  | **44.24**| **89.88**| **6.81**| **98.40**| 62.20| 84.16| **63.35**| 83.39| **64.82**| **80.46** |

[1] Ansuini et al. "Intrinsic dimension of data representations in deep neural networks." NeurIPS 2019.  
[2] Moayeri et al. "Text-to-concept (and back) via cross-model alignment." ICML 2023.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Official Review of Submission3444 by Reviewer kqnV


Firstly, we thank you for your thorough review of our paper. We particularly appreciate your recognition of our innovative approach using only textual data for hate detection, which eliminates the need to source hateful images and addresses ethical concerns. Additionally, we value your acknowledgment of our comprehensive experimentation, ablation analysis, and the provision of implementation details and code for reproducibility.

We are also immensely grateful for your excellent suggestions that can enhance the contents of our paper. We will address each of your concerns in detail in the following:

>**Q1**. The writing structure could be improved. The textual synthesis aspect is not clear to me and should be discussed in more detail in the main paper. 

**A1**. We apologize for any inconvenience caused in understanding our paper. In our method, the purpose of textual data synthesis is to emulate the entire visual dataset for training. We assumed that using prompt templates, such as "a photo of a {}", to generate text data could effectively emulate visual data, based on observations of high CLIP zero-shot classification performance with similar prompts. Therefore, our textual data synthesis involves simply inserting numerous words into the prompt "This is a photo of a {}". In our experiments, we used approximately 370k predefined English words. Our results demonstrate that even this lightweight textual data synthesis method can produce a detector capable of identifying various types of unwanted images.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

>**Q2**. The method could also be used for generic image classification tasks which brings me to question the choice of why such classification results have not been shown.

**A2**. In fact, our proposed method can always perform generic image classification and unwanted data detection simultaneously. Figure 1 in our paper or the figure in our repository (https://github.com/HFTT-anonymous/HFTT) can aid in understanding this. HFTT utilizes the input embeddings and logit values as they are for zero-shot classification while simultaneously estimating the probability that an input sample is unwanted. For example, our method can be applied to solve a 1001-class classification task consisting of 1000 ImageNet classes plus one OOD class.

However, applying our method does not enhance the zero-shot image classification performance of VLMs. This is because our method focuses solely on optimizing trainable embeddings for out-distribution detection while keeping CLIP frozen. Consequently, the image classification performance of VLMs remains the same as their zero-shot classification performance even after applying our method. Hence, we did not present classification results. For instance, the ImageNet classification accuracy of CLIP-ViT-B/16 remains at 68.6%, regardless of whether our method is applied.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

>**Q3**. Some more discussion over the baselines would be good too.

**A3**. Thank you for your suggestion. We provide further discussion on the strongest baselines and present results for various foundation models here:

**Comparison with SOTA OOD detection methods**  
NegLabel [1] and CLIPN [2] are cutting-edge OOD detection methods.
NegLabel constructs an OOD corpus by selecting texts distant from the in-distribution texts from a predefined corpus, then compares the distances between the input image and those texts in the CLIP embedding space to detect OOD. While NegLabel shows high OOD detection performance on ImageNet (see Table B), it has the following limitations compared to our method:
- Although NegLabel does not require training additional parameters, it must compute the embeddings of all texts in the corpus and measure their similarity to the in-distribution texts to find the optimal OOD corpus for a given in-distribution. Our training method also requires nearly the same cost as obtaining the embeddings of all texts within a predefined corpus and calculating the similarities between those embeddings and the task+trainable embeddings, as discussed in Section 4.1. Thus, NegLabel and our method require the same level of optimization cost.
- Since NegLabel uses the embeddings of the determined OOD corpus as they are, it falls behind our method, which has trainable parameters, in terms of generalization. To demonstrate this, we further compare our method and NegLabel in the medical image domain. Specifically, we treat the ISIC-18 skin lesion diagnosis dataset [3] as in-distribution and the PathVQA [4] and PatchCamelyon [5] datasets as out-of-distribution. The ISIC-18 skin lesion diagnosis dataset is an image classification benchmark for seven skin disease categories.

Table A: OOD detection in the medical image domain
|OOD:|PVQA||PCAM||
|-|-|-|-|-|
|**Method**|**FPR** &#8595;|**AUROC** &#8593;|**FPR** &#8595;|**AUROC** &#8593;|
|NegLabel|37.44|94.11|48.07|94.86|
|CLIPN|35.47|84.64|3.10|98.76|
|HFTT (ours)|13.72|97.05|4.95|98.35|

Table A illustrates the limitations of NegLabel in terms of generalization. While NegLabel fails to construct an effective OOD corpus for the medical image dataset, our method achieves significantly higher performance by learning optimal embeddings for detection.

CLIPN utilizes an additional "no" text encoder alongside CLIP. This additional text encoder predicts the probability that a given object is not present in an image. Thus, CLIPN predicts whether a given image is in-distribution or out-distribution by using the original CLIP text encoder and the "no" text encoder to estimate the probabilities, respectively. Images with a low probability of being in-distribution and a high probability of being out-distribution are identified as OOD.

Although CLIPN achieves high OOD detection performance on ImageNet (see Table B), it has the following limitations compared to our method:
- CLIPN requires significantly higher inference costs due to the use of an additional text encoder.
- While our method requires lightweight training that does not involve images, CLIPN demands extensive and expensive training of the "no" text encoder on large vision-language datasets.
- CLIPN can only be applied to tasks where the distinction between in-distribution and out-distribution is clear and straightforward, such as classification datasets. This is because all training images must be classified as either "yes" or "no" images. Therefore, it is unsuitable for tasks dealing with abstract concepts, such as hateful image detection, as discussed in Section 4.3 of our paper.
- Our method can be easily applied to any detection task defined in natural language, whereas CLIPN shows significantly degraded performance for in-distribution tasks that fall outside the training distribution of the "no" text encoder. In terms of applicability, our proposed method surpasses CLIPN. To demonstrate this, we further compare our method with CLIPN in the medical image domain. Table A illustrates the limitations of CLIPN in terms of generalization. While CLIPN effectively detects PCAM, it exhibits very low detection performance on PVQA. In contrast, our method achieves high performance on both OOD tasks.

Table B: OOD detection performance on ImageNet in-distribution (average for Texture, Places, SUN, and iNaturalist)
|OOD:| Average ||
|-|-|-|
|**Method**|**FPR** &#8595;|**AUROC** &#8593;|
|CLIPN|31.10|93.10|
|NegLabel|25.40|94.21|
|HFTT (ours)|33.33|91.76|

**Results for various foundation models**  
We provide the results for CLIP-L/14, BLIP-B/16, and BLIP-L/16 in addition to the CLIP-B/16 used in our study. Tables A, B, and C demonstrate that our method is effective across various vision-language models.

Table A: The experimental results on CLIP-L/14 (in-distribution: ImageNet)
|OOD:|iNaturalist||SUN||Places||Texture||NINCO|| 
|-|-|-|-|-|-|-|-|-|-|-|
|**Method**|**FPR** &#8595; |**AUROC** &#8593;|**FPR** &#8595;|**AUROC** &#8593;|**FPR** &#8595;| **AUROC** &#8593; |**FPR** &#8595;|**AUROC** &#8593;|**FPR** &#8595;|**AUROC** &#8593;|
|MSP|26.66|94.20|22.37|94.37|36.82|92.45|52.83|86.57|67.27|78.70|
|Energy|30.84|91.25|25.94|94.10|32.94|92.30|64.33|79.26|63.49|79.72|
|MaxLogit|32.76|90.96|26.48|92.96|**31.88**|92.39|72.08|73.85|**60.67**|**81.07**|
|MCM|64.41|26.96|94.19|22.77|94.37|36.74|92.44|52.66|86.56|68.16|78.65|
|HFTT (ours)|**24.10**|**94.58**|**17.80**|**95.39**|33.83|**93.09**|**52.06**|**86.58**|69.19|78.98|

Table B: The experimental results on BLIP-B/16 (in-distribution: ImageNet)
|OOD:|iNaturalist||SUN||Places||Texture||NINCO||
|-|-|-|-|-|-|-|-|-|-|-|
|**Method**|**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |
| MSP |  64.70 | 82.22 | 30.38 | 91.06 | 71.40 | 78.82 | 76.99 | 81.30 | **71.47** | 72.07   |
| Energy | 67.15 |  79.30 |  45.21 |  89.07 |  70.28  | 77.49 |  91.24 |  75.38 |  80.29  | **77.20**  |
| MaxLogit |  69.57 | 75.44 | 69.57 | 71.19 | 69.86 | 76.26 | 93.55 | 60.31 | 88.58 | 56.37 |
| MCM| 64.41  | **82.29** | 30.21 | 91.05 | 70.53 | 79.32 | 75.84 | 81.55 | 71.56 | 72.02  |
| HFTT (ours)    | **63.28** | 82.22 | **19.16** | **95.12** | **68.48** | **79.50** | **63.74** | **84.53** | 72.12 | 73.86   |

Table C: The experimental results on BLIP-L/16 (in-distribution: ImageNet)
| OOD:  | iNaturalist || SUN ||  Places || Texture || NINCO || 
|-|-|-|-|-|-|-|-|-|-|-|
|**Method**|**FPR** &#8595;| **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |**FPR** &#8595; | **AUROC** &#8593; |
| MSP |   51.20| 87.91| 22.37| 93.86| 61.63| 84.68| 64.85| 85.28| 65.96| 78.29 |
| Energy | 45.63 |87.23 |33.94 |90.29 |55.73 |85.91 |72.38 |82.16 |71.23| 77.49  |
| MaxLogit |  44.59| 86.94| 35.56| 86.45| **50.96**| **86.46**| 86.38| 71.22| 79.78| 67.59  |
| MCM| 50.75 |88.03 |22.34 |93.88 |60.88 |85.38 |64.71 |**85.39** |66.04| 78.32  |
| HFTT (ours)  | **44.24**| **89.88**| **6.81**| **98.40**| 62.20| 84.16| **63.35**| 83.39| **64.82**| **80.46** |

[1] Jiang et al. "Negative label guided ood detection with pretrained vision-language models." ICLR 2024.  
[2] Wang et al. "Clipn for zero-shot ood detection: Teaching clip to say no." ICCV 2023.  
[3] Codella, Noel, et al. "Skin lesion analysis toward melanoma detection 2018: A challenge hosted by the international skin imaging collaboration (isic)." arXiv 2019.  
[4] He, Xuehai, et al. "Pathvqa: 30000+ questions for medical visual question answering." arXiv 2020.  
[5] Veeling, Bastiaan S., et al. "Rotation equivariant CNNs for digital pathology." MICCAI 2018.

==> table/ablation_design_avg.tex <==
\begin{table}[]
\centering
\caption{Results of using different textual data synthesis methods. HFTT outperforms other methods that are more complex.}
\vspace{-0.3em}
\begin{tabular*}{0.75\columnwidth}{@{\extracolsep{\fill}}ccc@{}}
\toprule
Method & FPR&AUROC\\
\midrule[.05em]
WTO& 40.96& 88.30\\
CTO& 49.13& 83.29\\
DTO& 41.98& 88.02\\
Caption& 61.03& 75.66\\
Deduplication& 40.89& 88.33\\
HFTT (ours)& 40.72& 88.32\\
\midrule[.1em]

\end{tabular*}
% \vspace{-2.2em}
%\vskip -1mm
\label{tab:abl_design_avg}
\end{table}

==> table/ablation_focal_avg.tex <==
\begin{table}[h]
\centering
\caption{Results of using different values of $\gamma$ for the focal loss. The performance of HFTT appears to be relatively robust to changes in the choice of $\gamma$, with the adoption of focal loss with $\gamma > 0$ generally leading to improved results.}
\vspace{-0.3em}
{
\begin{tabular*}{0.5\columnwidth}{@{\extracolsep{\fill}}ccc@{}}
%\begin{tabular}{ccc}

\toprule
$\gamma$&FPR&AUROC\\
\midrule[.05em]
0& 41.18 & 88.19\\
1& 40.72 & 88.32\\
2& 40.58 & 88.31 \\
3& 40.61 & 88.29 \\
\midrule[.1em]
%\end{tabular}
\end{tabular*}
}
% \vspace{-1em}
\label{tab:abl_focal_avg}
\end{table}
